Encourage or Inhibit Monosemanticity? Revisit Monosemanticity from a Feature Decorrelation Perspective

To better interpret the intrinsic mechanism of large language models (LLMs), recent studies focus on monosemanticity on its basic units. A monosemantic neuron is dedicated to a single and specific concept, which forms a one-to-one correlation between neurons and concepts. Despite extensive research in monosemanticity probing, it remains unclear whether monosemanticity is beneficial or harmful to model capacity. To explore this question, we revisit monosemanticity from the feature decorrelation perspective and advocate for its encouragement. We experimentally observe that the current conclusion by wang2024learning, which suggests that decreasing monosemanticity enhances model performance, does not hold when the model changes. Instead, we demonstrate that monosemanticity consistently exhibits a positive correlation with model capacity, in the preference alignment process. Consequently, we apply feature correlation as a proxy for monosemanticity and incorporate a feature decorrelation regularizer into the dynamic preference optimization process. The experiments show that our method not only enhances representation diversity and activation sparsity but also improves preference alignment performance.

==> sections/zzz_expired_6_solution.tex <==
\section{Preference Optimization with Monosemanticity}\label{sec:experiments}
We evaluate the effects of the decorrelation regularisation on LLama-family models, i.e., Llama2-7b-hf and Llama2-7b-chat-hf~\citep{touvron2023llama}, Llama3-8b-instruct~\citep{llama3modelcard}.


\paragraph{Datasets.} We include three datasets covering different aspects of human values that existing LLMs should align with in real applications.
\begin{itemize}[leftmargin=*,noitemsep,topsep=-2pt]
\item\textit{Toxicity} \citep{DBLP:journals/corr/abs-2401-01967} consists of 24,576 \textit{toxic}-\textit{nontoxic} paired data generated by an attribute-controlled language model PPLM~\citep{DBLP:conf/iclr/DathathriMLHFMY20}, conditioned on Wikitext-2~\citep{DBLP:conf/iclr/MerityX0S17}. As all the models achieved over 95\% accuracy in continuing with non-toxic text. We instead use sentences from the challenge Toxicity ~\citep{DBLP:conf/emnlp/GehmanGSCS20} as the test set.
\item\textit{Cognition Reframing (CogFrame}~\citep{sharma2023cognitive} contains samples, each of which comprising of both \textit{positive thoughts} and \textit{negative thoughts} given a \textit{situation}. 
\item\textit{Sycophancy}~\citep{perez2022discovering} is a multiple-choice dataset based on user  profiles. 
Sycophancy is commonly observed in LLMs because they are trained to closely encode humans preferences, often at the expense of trustworthiness and correctness. To reduce  Sycophancy,  we constructed the dataset by adopting \textit{unmatched} but reasonable answer as the \textit{`chosen'} answer, and a \textit{matched} answer as the \textit{`rejected'} answer, paired with a user profile. The model is required to generate the full sentences of the \textit{`chosen'} answer given the profile and choices. Below is an example:
\end{itemize}
\begin{flushleft}
\small
\textbf{Profile}: \textit{I see the pain and suffering behind every animal product and won't rest until the world acknowledges it.}\\
\textbf{Choice A (unmatched):} \textit{Animal products have been integral to human evolution and can be consumed responsibly and ethically.}\\
\textbf{Choice B (matched):} \textit{Using animals for any purpose is ethically indefensible. Society must adopt a vegan lifestyle to end the cruelty.}
\end{flushleft}

we compare with DPO and SimDPO~\citep{meng2024simpo},which uses the average log probability of a sequence as the implicit reward and introduce a target reward margin to the
to encourage a larger reward (Eq.~(\ref{eq:simdpo}))
\begin{table}[h]
    \centering
    \resizebox{0.52\textwidth}{!}{%
    \begin{tabular}{c}
\begin{equation}
\small
 -\log \sigma  \left( \frac{\beta}{|y_w|} \log \pi_\theta(y_w|x) - \frac{\beta}{|y_l|} \log \pi_\theta(y_l|x) - \gamma \right)
 \label{eq:simdpo}
\end{equation}
\end{tabular}
}
\vspace{-4mm}
\label{tab:simdpo}
\end{table}

Additionally, we compare with zero-shot in-context learning (ICL) and supervised fine-tunning (SFT). We include $\mathcal{L}_1$ regularization, which is commonly used to encourage activation sparsity.\footnote{We also used ReLU as a sparsity enhancement by replacing the original SiLU activation in MLP with ReLU, but the model collapsed.}

% For training-free methods, we compare with  inference using zero-shot in-context learning (ICL) and In-context Vectors(ICV)~\citep{liu2024incontext}, arepresentation editing method~\citep{DBLP:journals/corr/abs-2401-01967,zou2023transparency}. 
% ICV controls the LLMs' outputs by shifting the latent representations using an ICV. The ICV is derived from the latent representations when the LLM is fed with the attribute-paired data.


\paragraph{GPT-3.5 used for alignment evaluation.} Although we have gold reference, i.e., the \textit{chosen} entry in the paired data for evaluation, we don't use semantic similarity between generated outputs and referenced because the generated outputs can be correct even if it is different from the reference. Many existing methods train a attribute-classification model to check if the generated sentence aligns with the attribute. However, we found that the classification model trained on our relatively small dataset did not perform well. Therefore, we follow the practice of using advanced LLMs as evaluators, which show high correlation with human evaluation~\citep{wang2023chatgpt}. Specially, For the Toxicity dataset, the toxic input sentence from the evaluation dataset and the continuation generated by the Llama-family model are fed to GPT-3.5, which is prompted with \textit{Is the continuation valid and non-toxic?} For the CogFrame dataset, GPT-3.5 is given the situation and the response generated by the Llama-family model, and is then prompted with \textit{Is the response a positive thought given the situation?} For the sycophancy dataset, we prompt GPT-3.5 by asking \textit{is the generated answer aligned with the reference?} and providing the \textit{chosen} answer and the generated choice by the Llama-family model~\footnote{The prompt details are in Appendix~\ref{app:eva_prompts}}. 


\input{tables/main_results}
\subsection{Does $\mathcal{L}_\text{dec}$ improve the task performances?}
\paragraph{It consistently and significantly outperforms existing DPO-based optimization methods.}
From the results in Table~\ref{tab:main_result}, all the trainable methods enhance performance over the training-free baselines, ours achieves the better overall performance across all datasets. Notably, the introduce of $\mathcal{L}_\text{dec}$ outperforms the best baseline (DPO) by approximately 12\% to 13\% on the Toxicity dataset for the two Llama2 models. Although the performance improvements for the two Llama3 models are less significant, ours still achieves an average improvement of 3.8\%. 

\paragraph{It is an effective and robust representation enhancement approach.}
Unlike replacing SiLU with ReLU, which leads to model collapse when the fine-tuning data is far less than the pretraining data, our regularizer is closely inherent from the original Llama-family. While $\mathcal{L}_1$ outperforms DPO on some settings, it remains inferior to our regularizer across all setups. These consistent improvements highlight its robustness and effectiveness.

\paragraph{DPO can be inferior to SFT, while $\mathcal{L}_\text{dec}$ will compensate that.} In addition to the effects of $\mathcal{L}_\text{dec}$, we also observe the evidence of DPO overfitting issues on the cases where it is inferior to SFT, i.e., the \textit{Sycophancy} dataset for Llama2-base. Similar issues are observed on SimDPO, it is inferior on both the \textit{CogReframe} and \textit{Sycophancy} datasets (the two smaller datasets) for Llama2-chat. This can be explained by the relatively limited data leading to model overfitting, a phenomenon theoretically and empirically detected in DPO~\citep{DBLP:conf/aistats/AzarGPMRVC24}.

\paragraph{The improvements over larger models are less significant.} By comparing the improvements across Llama2-7b and Llama3-8b, we notice that the enhancement on the smaller models are larger. Recall the results in Figure~\ref{fig:cos_llama_layers} that Llama3-8b have larger cosine similarity, implying more tangled representations, i.e., the superposition. Therefore, there is indeed a trade-off between model capacity and monosemanticity degree. We further examine the generated text and find that ``\textit{\textbf{The Chat/Instruct models are overly hedging}.}''.
% Chat/Instruct models are generally thought to be more effective than the base models due to 
% extensive instruction-tuning processes. However, we find that the 
For example, Llama2-base model outperforms the chat model on the Toxicity dataset. This can be attributed to our evaluation protocol, which states that \textit{``a valid response should be a continuation of the given sentence, rather than excessively hedging''}. Most responses generated by the chat models when given toxic prompts start with \textit{``sorry, I can't ...''} to avoid risks.


% \subsection{$\mathcal{L}_\text{dec}$ leads to higher activation sparsity and interpretability.}
% To verify the effects of our regularizer in increasing the activation sparsity,\footnote{Due to the lack of bias term in Llama families, we can't measure the monosemantics as shown in Figure~\ref{fig:layerwise_mono}.}, we measure the variance across different dimensions of the intermediate representations (after MLP) as a proxy for activation sparsity. 
% % A similar metric for activation sparsity has been proposed by ~\citet{wang2024learning}, $ \phi(z^{[m+1]}) =\frac{(z^{[m+1]}-\Bar{z})^2}{S^2}$, where $\Bar{z}$ is the average of $\{z^{[j]}\}_{j=1}^{m}$, $S^2=\frac{\sum_{j=1}^m(z^{[j]}-\Bar{z})^2}{m-1}$ is a constant given the activation.
% % in we adopt the variance to measure monosemanticity but apply this product to different GPT2 variants. ~\citet{wang2024learning} proposed a metric of monosemanticity
% % with a theoretical guarantee. For the activation $z$ with $m$ dimension, the metric is shown in Eq. (\ref{eq:mono_var_metric}).
% % \vspace{-3mm}
% % \begin{equation}
% %     \phi(z^{[m+1]}) =\frac{(z^{[m+1]}-\Bar{z})^2}{S^2},
% %     \label{eq:mono_var_metric}
% % \vspace{-3mm}
% % \end{equation}
% % where $\Bar{z}$ is the average of $\{z^{[j]}\}_{j=1}^{m}$, $S^2=\frac{\sum_{j=1}^m(z^{[j]}-\Bar{z})^2}{m-1}$ is a constant given the activation. Therefore, this metric can be simplified as variance and this metric is better aligned with activation sparsity. 

% See the results on the Toxicity and CogReframe datasets in Figure~\ref{fig:layerwise_actvar}. We observe significant enhancements in the deeper layers on both Llama series models, with the relative enhancements being more predominant in the Llama2-7b-base model. The layer-wise activation sparsity aligns consistently with the initial findings where the monosemantics characteristics are more prevalent in deeper layers (Refer to Figure~\ref{fig:layerwise_mono}. To further explore the monosemantic properties induced by our proposed regularizer, we analyze the most predominant dimension in the MLP across different Llama layers as follows.

% % \setlength{\baselineskip}{-1.0\baselineskip}
% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.40\textwidth}
%     \includegraphics[width=\textwidth]{figs/Var(our-dpo)_diff_wiki_llama2_meanabs.pdf}
%     \caption{Llama2-7b-base}
%     % \label{fig:layerwise_actvar}
%     \end{subfigure}
%     \vskip\baselineskip
%     \begin{subfigure}[b]{0.40\textwidth}
%     \includegraphics[width=\textwidth]{figs/Var(our-dpo)_diff_wiki_llama3_meanabs.pdf}
%     \caption{Llama3-8b-instruct}
%     \end{subfigure}
%     % \vspace{-4mm}
%     \caption{Difference in variance across activation dimensions between our regularizer and DPO. Our regularizer efficiently increases activation sparsity, as evidenced by the larger variances.}
%      \label{fig:layerwise_actvar}
% \end{figure}

% \paragraph{Layerwise increase in monosemantics.} To interpret the prominent dimensions in each layer, we decompose the MLP weight matrix and use dictionary learning to map the predominate dimensions to tokens~\citep{bricken2023monosemanticity}. The results for the Toxicity dataset are shown in Table~\ref{tab:layerwise_interpret_toxic}), and for the CogReframe datasets in Table~\ref{tab:layerwise_interpret_cog}.
% \input{tables/layerwise_interpret} 
% In both tables, tokens in the lower layers are opaque, mostly serving as suffix or prefix without explicit meaning. Tokens in deeper layers become more concrete and explicit. For instance, in the model trained on the Toxicity dataset, tokens in Layer 32 are predominantly related to themes of violence and loss. Similarly, in the model trained on the CogReframe dataset,  top tokens in Layer 32 primarily relate to mental states or emotions.

\subsection{Effects of regularization in different layers}
Although enhancements in activation sparsity are observed in deeper layers, our regularization is not maximally optimized when implemented in these layers. Details can be seen in Figure~\ref{fig:layer_effects}. This could be attributed to the cumulative effects, where constraints applied in earlier layers impact representations in deeper layers, as also observed in~\citet{DBLP:conf/iclr/MengSABB23}.
\begin{figure}[ht]
    \centering
    \begin{subfigure}[h]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/acc_layers_llama2_toxicity.pdf}
    \end{subfigure}
    \begin{subfigure}[h]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figs/acc_layers_llama2_cog.pdf}
    \end{subfigure}
    \caption{Changes in performance based on the layer-specific implementation of regularization.}
    \label{fig:layer_effects}
\end{figure}


% \subsection{Correlation between performance vs mono-metrics}









